Improving Robust Fairness via Balance Adversarial Training

Adversarial training (AT) methods are effective against adversarial attacks, yet they introduce severe disparity of accuracy and robustness between different classes, known as the robust fairness problem. Previously proposed Fair Robust Learning (FRL) adaptively reweights different classes to improve fairness. However, the performance of the better-performed classes decreases, leading to a strong performance drop. In this paper, we observed two unfair phenomena during adversarial training: different difficulties in generating adversarial examples from each class (source-class fairness) and disparate target class tendencies when generating adversarial examples (target-class fairness). From the observations, we propose Balance Adversarial Training (BAT) to address the robust fairness problem. Regarding source-class fairness, we adjust the attack strength and difficulties of each class to generate samples near the decision boundary for easier and fairer model learning; considering target-class fairness, by introducing a uniform distribution constraint, we encourage the adversarial example generation process for each class with a fair tendency. Extensive experiments conducted on multiple datasets (CIFAR-10, CIFAR-100, and ImageNette) demonstrate that our method can significantly outperform other baselines in mitigating the robust fairness problem (+5-10\% on the worst class accuracy)

==> resources/fig_5_cifar6.tex <==
\begin{figure}[h]
\centering
%
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/CIFAR10_wo2345.jpg}
\caption{Training w/o. class 2, 3, 4, 5}
\label{fig:CIFAR10_wo2345}
\end{subfigure}
%
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/CIFAR10_wo1689.jpg}
\caption{Training w/o. class 1, 6, 8, 9}
\label{fig:CIFAR10_wo1689}
\end{subfigure}
%
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/CIFAR10.jpg}
\caption{Training on all classes}
\label{fig:CIFAR10}
\end{subfigure}
%
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/CIFAR10_ours.jpg}
\caption{Training on all classes(ours)}
\label{fig:CIFAR10_ours}
\end{subfigure}
%
\caption{ 
The difference between training and test set during standard training and AT. Class 2,3,4 and 5 have poor previous performance.  Class 1,6,8 and 9 have good previous performance.} \label{fig:class}
\end{figure}


==> resources/fig_5_fairness.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.46\linewidth}
		\includegraphics[width=\textwidth,trim=150 5 5 5,clip]{figures/source_fairness.pdf}
		\caption{Source fairness}
		\label{fig:source_fairness}
\end{subfigure}
\begin{subfigure}[t]{0.46\linewidth}
		\includegraphics[width=\textwidth,trim=150 5 5 5,clip]{figures/target_fairness.pdf}
		\caption{Target fairness}
		\label{fig:target_fairness}
\end{subfigure}
\caption{
Source-class and Target-class fairness on BAT}
\label{fig:fairness}
%
\end{figure}
